Acoustic characteristics of supersonic planar impinging jets

The present work aims to study the tonal and broadband noise associated with a supersonic planar jet impinging on a flat plate. Five different cases are considered corresponding to different plate distance and angle of impingement. The near-field noise is analyzed using Large Eddy Simulation (LES). For this, we employ a low dispersive and dissipative Finite Volume solver using AUSM for inviscid fluxes and third order Runge-Kutta method for temporal discretization. The far-field noise is calculated using a hybrid approach in which the acoustic sources and mean flow are provided by the fluid solver while the far-field acoustic pressure is calculated by an acoustic solver. It solves Acoustic Perturbation Equations using a spectral/hp element method with a Discontinuous Galerkin projection. The present work highlights many important aspects of impinging jets. Firstly, the far-field sound with the effect of non-uniform base-fields is obtained which is important as the far-field acoustic pressure in most of the literature is reported either without any basefields or by the application of uniform base-fields. Secondly, a correlation between the different modes of oscillations of the impinging jet and the production of impinging tones is studied using Modal Decomposition techniques. This analysis also sheds some light on the number of concurrent cycles for different nozzle to plate distance. Lastly, the relation between the phase lag term and the distance between the plate and the nozzle exit is highlighted using a vortex tracking method. This observation can serve to provide a better understanding of the sound generation process.

==> figuresSYNTAXLATEX <==
\begin{figure}
	% include second image
	\includegraphics[scale=0.5]{FIGURES/TKE}  
	\caption{\label{fig:8}Turbulent Kinetic Energy profiles at different axial locations}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.58]{FIGURES/sourceBFS}% Here is how to import EPS art
	\caption{\label{fig:9} Vortex Source terms for Forward-Backward Facing Step: a) x-component of Lamb Vector, b) y-component of Lamb Vector}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.65]{FIGURES/pBFS}% Here is how to import EPS art
	\caption{\label{fig:10} Perturbation Pressure Distribution for Forward-Backward Facing Step}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/fftBFS}% Here is how to import EPS art
	\caption{\label{fig:11} SPL at 1m above the step}
\end{figure}
\begin{figure}
	\includegraphics[scale=0.6]{FIGURES/meshCWL}% Here is how to import EPS art
	\caption{\label{fig:12} a) Fluid Mesh, b) Acoustic Mesh for a cavity with a lip}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/sourceCWL}% Here is how to import EPS art
	\caption{\label{fig:13} Vortex Source terms for a cavity with a lip: a) x-component of Lamb Vector, b) y-component of Lamb Vector }
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/pCWL}% Here is how to import EPS art
	\caption{\label{fig:14} Perturbation Pressure for a cavity with a lip }
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/fftCWL}% Here is how to import EPS art
	\caption{\label{fig:15} Pressure spectrum for a cavity with a lip }
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/CAVMESH}% Here is how to import EPS art
	\caption{\label{fig:16} a) Fluid Mesh, b) Acoustic mesh for Subsonic Cavity}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.4]{FIGURES/FFTMpt7}% Here is how to import EPS art
	\caption{\label{fig:17} SPL for cavity at M = 0.7 at x/D=-0.04,y/D=2}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.4]{FIGURES/PLINEFINAL}% Here is how to import EPS art
	\caption{\label{fig:18} Pressure perturbation along the line $x+y=2D$; $r=\sqrt{x^2 + y^2}$}
\end{figure}
\begin{figure}
	\includegraphics[scale=0.6]{FIGURES/sourceMpt7}% Here is how to import EPS art
	\caption{\label{fig:19} Source terms for M = 0.7; a) x-component of Lamb Vector, b) y-component of Lamb Vector, c) Entropy Source term}
\end{figure}
\begin{figure}
	\includegraphics[scale=0.6]{FIGURES/pMpt7}% Here is how to import EPS art
	\caption{\label{fig:20} Pressure perturbation contours for M = 0.7}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/DIRMpt7}% Here is how to import EPS art
	\caption{\label{fig:21} Farfield Sound directivity for M = 0.7, $f=31.73kHz$, with $SPL(dB)$}
\end{figure}
\begin{figure}
	\includegraphics[scale=0.6]{FIGURES/sourceMpt6}% Here is how to import EPS art
	\caption{\label{fig:22} Source terms for M = 0.6; a) x-component of Lamb Vector, b) y-component of Lamb Vector, c) Entropy Source term}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/pMpt6}% Here is how to import EPS art
	\caption{\label{fig:23} Pressure perturbation contours for M = 0.6}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/DIRMpt6}% Here is how to import EPS art
	\caption{\label{fig:24} Farfield Sound directivity for M = 0.6, $f=28.1kHz$, with $SPL(dB)$}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/sourceMpt5}% Here is how to import EPS art
	\caption{\label{fig:25} Source terms for M = 0.5; a) x-component of Lamb Vector, b) y-component of Lamb Vector, c) Entropy Source term}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/pMpt5}% Here is how to import EPS art
	\caption{\label{fig:26} Pressure perturbation contours for M = 0.5}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/DIRMpt5}% Here is how to import EPS art
	\caption{\label{fig:27} Farfield Sound directivity for M = 0.5, $f=25.4kHz$, with $SPL(dB)$}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/sourceMpt4}% Here is how to import EPS art
	\caption{\label{fig:28} Source terms for M = 0.4; a) x-component of Lamb Vector, b) y-component of Lamb Vector, c) Entropy Source term}
\end{figure}
\begin{figure}
	\includegraphics[scale=0.6]{FIGURES/pMpt4}% Here is how to import EPS art
	\caption{\label{fig:29} Pressure perturbation contours for M = 0.4}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/DIRMpt4}% Here is how to import EPS art
	\caption{\label{fig:30} Farfield Sound directivity for M = 0.4, $f=22.0kHz$, with $SPL(dB)$}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/CAVMESHSUP}% Here is how to import EPS art
	\caption{\label{fig:31} a) Fluid Mesh, b) Acoustic Mesh for M = 1.5}
\end{figure}
\begin{figure}
	\includegraphics[scale=0.6]{FIGURES/fftM1p5}% Here is how to import EPS art
	\caption{\label{fig:32} SPL for the cavity at M = 1.5 at $x/D=-0.04, y/D=2$}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.6]{FIGURES/sourceM1p5}% Here is how to import EPS art
	\caption{\label{fig:33} Source terms for M = 1.5; a) x-component of Lamb Vector, b) y-component of Lamb Vector, c) Entropy Source term}
\end{figure}
\begin{figure}	
	\includegraphics[scale=0.9]{FIGURES/pM1p5}% Here is how to import EPS art
	\caption{\label{fig:34} Pressure perturbation for M = 1.5}
\end{figure}
\begin{figure}
	\begin{subfigure}{1\textwidth}
		% include first image
		\includegraphics[scale=0.6]{FIGURES/IntSource1}  
		\caption{vortex clipping}
		\label{fig:35(a)}
	\end{subfigure}
	
	\begin{subfigure}{1\textwidth}
		% include second image
		\includegraphics[scale=0.6]{FIGURES/IntSource2}  
		\caption{New vortex from the leading edge}
		\label{fig:35(b)}
	\end{subfigure}
\end{figure}
\begin{figure}
	\ContinuedFloat
	\begin{subfigure}{1\textwidth}
		% include second image
		\includegraphics[scale=0.6]{FIGURES/IntSource3}  
		\caption{Vortex bending}
		\label{fig:35(c)}
	\end{subfigure}
	
	\begin{subfigure}{1\textwidth}
		% include second image
		\includegraphics[scale=0.6]{FIGURES/IntSource4}  
		\caption{New vortex clipping}
		\label{fig:35(d)}
	\end{subfigure}
	\caption{Evolution of sources for subsonic cavity flow}
	\label{fig:35}
\end{figure}
\begin{figure}
	\begin{subfigure}{1\textwidth}
		% include first image
		\includegraphics[scale=0.6]{FIGURES/IntSource6}  
		\caption{vortex pair at the leading edge}
		\label{fig:36(a)}
	\end{subfigure}
	\begin{subfigure}{1\textwidth}
		% include second image
		\includegraphics[scale=0.6]{FIGURES/IntSource7}  
		\caption{vortex clipping at the trailing edge}
		\label{fig:36(b)}
	\end{subfigure}
\end{figure}
\begin{figure}
	\ContinuedFloat
	\begin{subfigure}{1\textwidth}
		% include second image
		\includegraphics[scale=0.6]{FIGURES/IntSource8}  
		\caption{Discrete vortices at the leading edge}
		\label{fig:36(c)}
	\end{subfigure}
	\begin{subfigure}{1\textwidth}
		% include second image
		\includegraphics[scale=0.6]{FIGURES/IntSource9}  
		\caption{Merging of vortices}
		\label{fig:36(d)}
	\end{subfigure}
\end{figure}
\begin{figure}
	\ContinuedFloat
	\begin{subfigure}{1\textwidth}
		% include second image
		\includegraphics[scale=0.6]{FIGURES/IntSource10}  
		\caption{vortex bending}
		\label{fig:36(e)}
	\end{subfigure}
	\caption{Evolution of sources for supersonic cavity flow}
	\label{fig:36}
\end{figure}  
